Assessing incrementality in sequence-to-sequence models

Since their inception, encoder-decoder models have successfully been applied to a wide array of problems in computational linguistics. The most recent successes are predominantly due to the use of different variations of attention mechanisms, but their cognitive plausibility is questionable. In particular, because past representations can be revisited at any point in time, attention-centric methods seem to lack an incentive to build up incrementally more informative representations of incoming sentences. This way of processing stands in stark contrast with the way in which humans are believed to process language: continuously and rapidly integrating new information as it is encountered. In this work, we propose three novel metrics to assess the behavior of RNNs with and without an attention mechanism and identify key differences in the way the different model types process sentences.

==> novel_models.tex <==
\subsection{Novel models}\label{sec:novel}

\citeauthor{christiansen2016now} \cite{christiansen2016now} identify several components which either make up or are implications of their hypothesized \emph{Now-or-Never bottleneck}, a set
of fundamental contraints on human language processing, which include a limited amount of available memory and time pressure. To ensure a successful processing of language, the human brain seems to be forced to anticipate future utterances and employ a lossy compression of inputs as soon as they are encountered as well as encoding them into more and more abstract representations, which seems highly reminiscent of the encoder in today's encoder-decoder architectures. We try to realize these components in new models, which are described in the following sections.

\subsubsection{Anticipation Loss}\label{sec:anticipation_loss}

\citeauthor{christiansen2016now} \cite{christiansen2016now} describe anticipation, realized in a mechanism called \emph{predictive processing} as one of the implications of the Now-or-Never bottleneck: As humans have to process a sequence of inputs fast, they already try to anticipate the next element before it is being uttered. This seems to be the reason why people struggle with so-called garden path sentences like ``The horse race past the barn fell", where the last word encountered, ``fell'', goes against the representation of the sentence built up until this point.

To incentivize an encoder to anticipate future tokens, we augment the training objective with a language modeling loss we call \emph{Anticipation Loss}. To that end, the current encoder hidden state $\bh_t$ is projected into vocabulary space and then used to compute the cross-entropy loss between the resulting distribution over words and the actual, next occuring word:

\begin{equation}
  \mathbf{\tilde{a}}_t = \mathbf{W}_{antcp}\bh_t + \mathbf{b}_{antcp}
\end{equation}
\begin{equation}
  \mathbf{a}_t = softmax(\mathbf{\tilde{a}}_t)
\end{equation}

were $\mathbf{\tilde{a}}_t, \mathbf{a}_t \in \mathbb{R}^{|V|}$ with $V$ being the set of all words in the vocabulary and

\begin{equation}
  \mathcal{L}_{antcp} = - \frac{1}{T-1}{\displaystyle \sum_{t=1}^{T-1}}{\displaystyle \sum_{i=1}^{|V|}}\delta(i, t+1)\log(\mathbf{a}_{ti})
\end{equation}

where $\delta(i, t+1) = 1$ if vocabulary entry $V_i$ corresponds to the next token $x_{t+1}$ and $0$ otherwise.

\subsubsection{Bottleneck Decoder}\label{sec:bottleneck_decoder}

Another strategy being employed by humans in processing language seems to be \emph{eager processing}; the cognitive system encodes new input into ``rich'' representations as fast as possible. To enforce some temporal pressure on the
decoder so that the encoder is forced to create better representations to compensate for the decoder's lack of total access to all its encodings, we mask
the attention weights $\alpha_{it}$ of the decoder in two distinct ways: 1. We mask all the
hidden representations that occur after the current \emph{decoder} time step (the
decoder only has access to past encoded inputs) with a vector $\mathbf{m}_i$:

\begin{equation}
    \mathbf{m}_i = [\delta_{i \ge 1}, \ldots, \delta_{i \ge T}]^T
\end{equation}

where $\delta$ denotes \emph{Kronecker's delta}.

 2. We only give the decoder access
to a number of representations around the current decoder time step with a fixed
window size $w$. In the case of a window size of $1$ and a decoding time step of $t=2$
for example, all attention weights except for hidden states $\bh_1, \bh_2, \bh_3$
are masked. A similar idea has already been described by \cite{luong2015effective} as ``local attention''.

